Modeling the process of speciation using a multi-scale framework including error estimates

This paper concerns the modeling and numerical simulation of the process of speciation. In particular, given conditions for which one or more speciation events within an ecosystem occur, our aim is to develop the necessary modeling and simulation tools. Care is also taken to establish a solid mathematical foundation on which our modeling framework is built. This is the subject of the first half of the paper. The second half is devoted to developing a multi-scale framework for eco-evolutionary modeling, where the relevant scales are that of species and individual/population, respectively. Hence, a system of interacting species can be described at the species level, while for branching species a population level description is necessary. Our multi-scale framework thus consists of coupling the species and population level models where speciation events are detected in advance and then resolved at the population scale until the branching is complete. Moreover, since the population level model is formulated as a PDE, we first establish the well-posedness in the time-discrete setting, and then derive the a posteriori error estimates which provides a fully computable upper bound on an energy-type error, including also for the case of general smooth distributions (which will be useful for the detection of speciation events). Several numerical tests validate our framework in practice.

==> manuscript_clean _nored_nolineno/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{color}
\newcommand{\red}{\textcolor{red}}

\usepackage{subcaption}

\newcommand{\vecc}{\mathbf{c}}
\newcommand{\id}{{\mathbb I}}
\newcommand{\tol}{\textnormal{TOL}}
\newcommand{\real}{{\mathbb R}}
\newcommand{\dx}{\textnormal{d}x}
\newcommand{\textn}[1]{\textnormal{#1}}
\newcommand{\pt}{\partial_t}
\newcommand{\dy}{\textnormal{d}y}
\newcommand{\dzeta}{\textnormal{d}\zeta}
\newcommand{\bse}{\begin{subequations}}
\newcommand{\ese}{\end{subequations}}

\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\Cbb}{{\mathbb C}}
\newcommand{\Dbb}{{\mathbb D}}

\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Zcal}{\mathcal{Z}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Dcal}{\mathcal{D}}

\newcommand{\sigmabo}{\boldsymbol{\sigma}}
\newcommand{\Sigmabo}{\boldsymbol{\Sigma}}

\newcommand{\vecV}{\mathbf{V}}
\newcommand{\vecN}{\mathbf{N}}
\newcommand{\vecX}{\mathbf{X}}

\newcommand{\dnabla}{\nabla \nabla}
\newcommand{\dnablaii}{\nabla_i \nabla_i}
\newcommand{\dnablajj}{\nabla_j \nabla_j}
\newcommand{\dnablaij}{\nabla_i \nabla_j}

\newcommand{\vertiii}[1]{{\vert\kern-0.25ex\vert\kern-0.25ex\vert #1 \vert\kern-0.25ex\vert\kern-0.25ex\vert}}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\bnorm}[1]{\Big\lVert#1\Big\rVert}

\newcommand{\Hdiv}{\mathbf{H}(\divvv,\Omega)}
\newcommand{\divvv}{{\textnormal{div}}}

\newcommand{\etaRK}{\eta_{\textnormal{R},K}}
\newcommand{\etaDF}{\eta_{\textnormal{DF},K}}
\newcommand{\etaphih}{\eta_{\Phi}}
\newcommand{\etagh}{\eta_{g,K}}
\newcommand{\etarh}{\eta_{r,K}}
\newcommand{\etaosch}{\eta_{f}}
\newcommand{\etaphihj}{\eta_{\Phi,i}}

\newcommand{\etaRKj}{\eta_{\textnormal{R},K,i}}
\newcommand{\etaDFj}{\eta_{\textnormal{DF},K,i}}
\newcommand{\etaghj}{\eta_{g,K,i}}
\newcommand{\etarhj}{\eta_{r,K,i}}

\newcommand{\dist}{\textnormal{dist}}
%%%%%%%%%%%%%%%%%%%%%%%%


% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

%%
\newsiamthm{assum}{Assumption}
\newsiamthm{df}{Definition}
%%

% Sets running headers as well as PDF title and authors
\headers{Modeling the process of speciation using a multi-scale framework}{M. K. Brun, E. Ahmed, J. M. Nordbotten, and N. C. Stenseth}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Modeling the process of speciation using a multi-scale framework including a posteriori error estimates\thanks{Submitted to the editors DATE.
\funding{This work was funded 
in part by Norwegian Research Council project no.~263149.}}}

% Authors: full names plus addresses.
\author{
	Mats K. Brun\thanks{CEES, Dept. of Biosciences, University of Oslo, NO-0316 Oslo, Norway. Current address: Expert Analytics, NO-0179 Oslo, Norway 
  			(\email{m.k.brun@ibv.uio.no}/\email{mats@xal.no}).} 
	\and Elyes Ahmed\thanks{SINTEF, NO-0314 Oslo, Norway 
  			(\email{elyes.ahmed@sintef.no}).}
	\and Jan M. Nordbotten\thanks{Department of Mathematics, University of Bergen, NO-5020 Bergen, Norway 
  			(\email{jan.nordbotten@uib.no}).}
	\and Nils Chr. Stenseth\thanks{CEES, Dept. of Biosciences, University of Oslo, NO-0316 Oslo, Norway 
  			(\email{n.c.stenseth@mn.uio.no}).}
}
\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

